From Data to Insights: A Covariate Analysis of the IARPA BRIAR Dataset for Multimodal Biometric Recognition Algorithms at Altitude and Range

This paper examines covariate effects on fused whole body biometrics performance in the IARPA BRIAR dataset, specifically focusing on UAV platforms, elevated positions, and distances up to 1000 meters. The dataset includes outdoor videos compared with indoor images and controlled gait recordings. Normalized raw fusion scores relate directly to predicted false accept rates (FAR), offering an intuitive means for interpreting model results. A linear model is developed to predict biometric algorithm scores, analyzing their performance to identify the most influential covariates on accuracy at altitude and range. Weather factors like temperature, wind speed, solar loading, and turbulence are also investigated in this analysis. The study found that resolution and camera distance best predicted accuracy and findings can guide future research and development efforts in long-range/elevated/UAV biometrics and support the creation of more reliable and robust systems for national security and other critical domains.

==> supplimental.tex <==

\newpage

%------------------------------------------------------------------------
\section*{Supplemental Material}

\begin{table*}[h]
    \centering
\begin{tabular}{lllll}
\hline
algorithm tag & developer & name & version & results \\
\hline
System A & Systems Technology Research & Str Morfius & 2.2.3 &  \\
System B & Michigan State University & humanid & 3.8.1 &  \\
System C & Kitware & Kitware DOERS BRIAR Service & 2.1.0 &  \\
System D & Accenture Federal Services & AFSBLAU & 2.9.3 &  \\
System E & University of Southern California & GrailService.v2.0 & 2.0.0 &  \\
\hline
\end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}


\begin{table*}[h]
    \centering
\begin{tabular}{ll}
\hline
Evaluation Protocol Summary &  \\
\hline
Evaluation Protocol Version & 4.2.1 \\
Evaluation Phase & 2 \\
Probe Set & main \\
Gallery Type & simple \\
\hline
\end{tabular}

    \caption{Caption}
    \label{tab:my_label}
\end{table*}



\begin{table*}[h]
    \centering
\begin{tabular}{lllll}
\hline
 & 0 & 1 & 2 & 3 \\
\hline
0 & Model: & MixedLM & Dependent Variable: & est far \\
1 & No. Observations & 41119 & Method & REML \\
2 & No. Groups: & 55 & Scale: & 4.3539 \\
3 & Min. group size: & 30 & Log-Likelihood: & -88768.7911 \\
4 & Max. group size: & 3185 & Converged: & Yes \\
5 & Mean group size: & 747.6 &  &  \\
\hline
\end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}


\begin{table*}
    \centering
\begin{tabular}{lllllll}
\hline
Cov.Name & Level & Coef. & [0.025 & 0.975] & P>|z| & Num.Probes \\
\hline
Intercept & - & -7.003 & -7.340 & -6.666 & 0.000 & - \\
Algorithm & System A & 0.000000 & 0 & 0 & - & 8245 \\
Algorithm & System B & 0.273 & 0.210 & 0.337 & 0.000 & 8213 \\
Algorithm & System C & 0.447 & 0.383 & 0.511 & 0.000 & 8230 \\
Algorithm & System D & 0.692 & 0.628 & 0.756 & 0.000 & 8237 \\
Algorithm & System E & 0.407 & 0.343 & 0.471 & 0.000 & 8194 \\
Has Gait & False & 0.000000 & 0 & 0 & - & 24804 \\
Has Gait & True & -0.283 & -0.332 & -0.233 & 0.000 & 0 \\
Has Turb. & False & 0.000000 & 0 & 0 & - & 27586 \\
Has Turb. & True & 0.057 & -0.012 & 0.127 & 0.104 & 0 \\
Head Height & >90 Pix & 0.000000 & 0 & 0 & - & 11388 \\
Head Height & 60-90 Pix & 0.480 & 0.384 & 0.576 & 0.000 & 3473 \\
Head Height & 50-60 Pix & 0.516 & 0.406 & 0.625 & 0.000 & 3293 \\
Head Height & 40-50 Pix & 0.673 & 0.576 & 0.771 & 0.000 & 7253 \\
Head Height & 30-40 Pix & 1.322 & 1.216 & 1.428 & 0.000 & 4581 \\
Head Height & <30 Pix & 1.884 & 1.730 & 2.038 & 0.000 & 1290 \\
Head Height & Restricted & 2.232 & 2.151 & 2.313 & 0.000 & 9841 \\
Modality & Face & 0.000000 & 0 & 0 & - & 10525 \\
Modality & Body & 0.742 & 0.642 & 0.842 & 0.000 & 30594 \\
Camera Location & Ctrl & 0.000000 & 0 & 0 & - & 7392 \\
Camera Location & Short Range & -0.344 & -0.489 & -0.200 & 0.000 & 2155 \\
Camera Location & Medium Range & 0.949 & 0.792 & 1.106 & 0.000 & 10472 \\
Camera Location & Long Range & 1.952 & 1.716 & 2.187 & 0.000 & 9673 \\
Camera Location & Elevated & 0.214 & 0.109 & 0.318 & 0.000 & 10510 \\
Camera Location & Uav & 0.999 & -0.122 & 2.120 & 0.081 & 917 \\
Solar Loading & 0-300 W/M$^2$ & 0.000000 & 0 & 0 & - & 19375 \\
Solar Loading & 300-600 W/M$^2$ & -0.199 & -0.266 & -0.132 & 0.000 & 7404 \\
Solar Loading & 600-900 W/M$^2$ & 0.511 & 0.434 & 0.588 & 0.000 & 7024 \\
Solar Loading & Above 900 W/M$^2$ & 0.868 & 0.791 & 0.945 & 0.000 & 7316 \\
Wind Speed & 0-3 M/S & 0.000000 & 0 & 0 & - & 25929 \\
Wind Speed & 3-6 M/S & -0.156 & -0.213 & -0.099 & 0.000 & 12453 \\
Wind Speed & 6-9 M/S & -0.043 & -0.145 & 0.059 & 0.412 & 2432 \\
Wind Speed & 9-12 M/S & 0.265 & 0.013 & 0.516 & 0.039 & 305 \\
Temperature & Below 0 C & 0.000000 & 0 & 0 & - & 4059 \\
Temperature & 0-10 C & 0.114 & 0.031 & 0.197 & 0.007 & 8327 \\
Temperature & 10-20 C & 0.333 & 0.185 & 0.481 & 0.000 & 8178 \\
Temperature & 20-30 C & -0.342 & -0.501 & -0.183 & 0.000 & 17684 \\
Temperature & 30-40 C & -0.143 & -0.329 & 0.043 & 0.132 & 2871 \\
Group Var & - & 1.157 &  &  &  & - \\
\hline
\end{tabular}

    \caption{Caption}
    \label{tab:my_label}
\end{table*}


\begin{table*}
    \centering

\begin{tabular}{lr}
\hline
 & count \\
group &  \\
\hline
DWC-MPTZ336XW - BGC3 & 3185 \\
acA2040-90um - BGC4 & 2175 \\
DWC-MPTZ336XW - BGC1 & 2025 \\
HDZP252DI - BGC3 & 1875 \\
acA2040-120uc - BGC2 & 1601 \\
XNZ-6320 - BGC3 & 1591 \\
acA2040-120uc - BGC1 & 1535 \\
HDZP252DI - BGC1 & 1490 \\
MPT-50 - BGC4 & 1465 \\
acA2040-120uc - BGC4 & 1429 \\
Q6215-LE - BGC4 & 1427 \\
PNP-9200RH - BGC2 & 1315 \\
HDZP252DI - BGC2 & 1303 \\
HDZP252DI - BGC4 & 1182 \\
MPT-90 - BGC2 & 1074 \\
acA2040-120um - BGC2 & 1060 \\
PNP-9200RH - BGC3 & 1055 \\
DWC-MPTZ336XW - BGC2 & 965 \\
acA2040-120uc - BGC3 & 911 \\
acA4112-30um - BGC4 & 848 \\
acA4112-30um - BGC3 & 771 \\
XNZ-6320 - BGC4 & 733 \\
XNZ-6320 - BGC2 & 721 \\
Q6215-LE - BGC2 & 680 \\
acA2040-90um - BGC2 & 644 \\
acA4112-30um - BGC1 & 610 \\
PNP-9200RH - BGC1 & 605 \\
Q6215-LE - BGC3 & 525 \\
Q6215-LE - BGC1 & 505 \\
QNP-6230H - BGC3 & 480 \\
P5655-E - BGC4 & 470 \\
Anafi - BGC1 & 465 \\
QNP-6230H - BGC4 & 450 \\
DWC-MPTZ336XW - BGC1.1 & 420 \\
HDZP252DI - BGC1.1 & 370 \\
P5655-E - BGC2 & 365 \\
XNZ-6320 - BGC1.1 & 284 \\
DWC-MPTZ336XW - BGC4 & 275 \\
Anafi USA - BGC1 & 250 \\
acA2040-90uc - BGC1 & 245 \\
MIC-IP-FUSION-9000IV - BGC4 & 220 \\
MPT-90 - BGC3 & 205 \\
PNP-9200RH - BGC4 & 195 \\
Anafi USA - BGC1.1 & 172 \\
Q6215-LE - BGC1.1 & 170 \\
PNP-9200RH - BGC1.1 & 165 \\
acA2040-120um - BGC1.1 & 123 \\
MIC-IP-FUSION-9000IV - BGC2 & 105 \\
P5655-E - BGC3 & 75 \\
acA2040-120um - BGC3 & 75 \\
P5655-E - BGC1.1 & 65 \\
acA2040-120uc - BGC1.1 & 55 \\
acA2040-90uc - BGC1.1 & 50 \\
a2A5328-15ucPRO - BGC3 & 35 \\
Mantis i45 EO - BGC1.1 & 30 \\
\hline
\end{tabular}

    \caption{Caption}
    \label{tab:my_label}
\end{table*}



